Reconstruction under outliers for Fourier-sparse functions

We consider the problem of learning an unknown $f$ with a sparse Fourier spectrum in the presence of outlier noise. In particular, the algorithm has access to a noisy oracle for (an unknown) $f$ such that (i) the Fourier spectrum of $f$ is $k$-sparse; (ii) at any query point $x$, the oracle returns $y$ such that with probability $1-\rho$, $|y-f(x)| \le \epsilon$. However, with probability $\rho$, the error $y-f(x)$ can be arbitrarily large. We study Fourier sparse functions over both the discrete cube $\{0,1\}^n$ and the torus $[0,1)$ and for both these domains, we design efficient algorithms which can tolerate any $\rho<1/2$ fraction of outliers. We note that the analogous problem for low-degree polynomials has recently been studied in several works~[AK03, GZ16, KKP17] and similar algorithmic guarantees are known in that setting. While our main results pertain to the case where the location of the outliers, i.e., $x$ such that $|y-f(x)|>\epsilon$ is randomly distributed, we also study the case where the outliers are adversarially located. In particular, we show that over the torus, assuming that the Fourier transform satisfies a certain \emph{granularity} condition, there is a sample efficient algorithm to tolerate $\rho =\Omega(1)$ fraction of outliers and further, that this is not possible without such a granularity condition. Finally, while not the principal thrust, our techniques also allow us non-trivially improve on learning low-degree functions $f$ on the hypercube in the presence of adversarial outlier noise. Our techniques combine a diverse array of tools from compressive sensing, sparse Fourier transform, chaining arguments and complex analysis.

==> LP_decoding.tex <==
\section{Linear Program Decoding for random outliers}\label{sec:linear_program_dec}
Given a domain $D$, a set $T$ of Fourier characters of $D$ and an oracle (with random outlier noise) to a  function $f$ supported 
on $k$ of these $T$ characters, we provide an algorithm with running time polynomial in $|T|$ which recovers $f$ (with small error). 
\begin{theorem}\label{thm:LP_guarantee_boolean_cube}
There is an algorithm which when given as input, sparsity parameter $k$, domain $D$, a set $T$ of Fourier characters over $D$, failure probability $\gamma$, parameters $\delta>0$ and $\eta>0$, and an oracle to $f=\sum_{j=1}^k \wh{f}(\xi_j) \cdot \chi_{j}$ (with each $\chi_j \in T$ and  $|\wh{f}(\xi_j)| \ge \eta$) with $( \frac{1}{2}-\delta, \eps)$ random outlier noise (where $\eps \lesssim \eta \cdot \delta$), makes $\tilde{O}(k^2 \log |T| \log \frac{1}{\gamma}/\delta^2)$ queries and runs in time $\poly(|T|, 1/\delta,1/\eta,\log \frac{1}{\gamma})$ and 
outputs $g$ satisfying 
$$
\supp(\wh{g})=\supp(\wh{f}) \text{ and } |\wh{g}(\xi)-\wh{f}(\xi)| \lesssim \frac{\epsilon}{\delta} \text{ for every } \xi,$$   with probability  $1-\gamma.$
\end{theorem}
The algorithm is described in Algorithm~\ref{alg:LP_decoding_boolean} and we prove its correctness in the rest of this section. To do so, we will consider the following optimization problem (which can be easily formulated as a linear program). In particular, suppose the observations at points $x_1, \ldots, x_m$ are $y(x_1), \ldots, y(x_m)$ respectively. Further, for $1 \le i \le m$, define $e(x_i) = y(x_i) -f(x_i)$ be the noise at point $i$ and let $\Delta$ be an estimate of this noise, i.e, $\sum_{i=1}^m |e(x_i)|$. Then, the optimization problem (where $\{g(x)\}_{x \in D}$ are the unknowns) is 
\begin{equation}\label{eq:LP_decode_sparseFFT}
\min \|\wh{g}\|_1 \quad \text{ subject to } \sum_{i=1}^m |g(x_i)-y(x_i)| \le \Delta \text{ and } g \in \text{span}\{T\}.
\end{equation}
It is easy to see that (\ref{eq:LP_decode_sparseFFT}) can be formulated as a linear program. Algorithm~\ref{alg:LP_decoding_boolean} is described next. 
\begin{algorithm}[H]
\caption{Linear Program Decoding for sparse FFT}\label{alg:LP_decoding_boolean}
\begin{algorithmic}[1]
\Procedure{\textsc{LinearDecodingSparseFFT}}{$y,T,k,\gamma,\delta,\eta$}
\State $m:=\tilde{O}\bigg( k^2 \log |T| \log \frac{1}{\gamma} /\delta^2 \bigg)$ 
\State Sample $m$ random points $x_1,\ldots,x_m$ and let $y(x_1),\ldots,y(x_m)$ be the corresponding observations. 
\State $\sigma:=m \cdot \frac{\eta \cdot \delta}{100}$
\For{$\Delta$ from 0 to $\sum_i |y(x_i)| + \eta m$ with gap $\sigma$}
\State Solve the linear program \eqref{eq:LP_decode_sparseFFT} to obtain $g$ given $\Delta$, $T$, and $x_1,\ldots,x_m$ with the corresponding observations $y(x_1),\ldots,y(x_m)$.
\State Set $S_{\Delta}=\{\textit{The $k$ characters in $g$ with the largest absolute coefficients}\}$.
\State Let $g_{\Delta}=\underset{h \in \text{span}(S_{\Delta}) }{\arg\min} \sum_{i=1}^m |h(x_i)-y(x_i)|$.
\EndFor
\\
\Return $g=\underset{g_{\Delta}}{\arg\min} \sum_{i=1}^m |g_{\Delta}(x_i)-y(x_i)|$.
\EndProcedure
\end{algorithmic}
\end{algorithm}
First notice that under the assumption $\|y\|_{\infty} \le \poly(k)$, our algorithm runs in time $\poly(k,|T|,1/\eta,1/\delta,\log \frac{1}{\gamma})$.
In the rest of this section, we only consider $h:D \rightarrow \mathbb{R}$ whose Fourier transform is supported on  $T$ and let $\|\wh{h}\|_1$ and $\|\wh{h}\|_2$ denote $\sum_{\chi \in T} |\wh{h}(\chi)|$ and $\big( \sum_{\chi \in T} |\wh{h}(\chi)|^2 \big)^{1/2}$ separately. We next show the following  guarantee for the LP \eqref{eq:LP_decode_sparseFFT}.
\begin{lemma}\label{lem:guarantee_LP}
For any failure probability $\gamma$, parameters $\delta>0,$ and $\eps>0$ , define $\rho=1/2-\delta$ and $m=\tilde{O} \bigg( k^2 \log |T| \log \frac{1}{\gamma}/\delta^2 \bigg)$. Let $f: D \rightarrow \mathbb{R}$ be such that $\|\wh{f}\|_0 \le k$ and for any point $x$, let $y(x)$ be the output of an oracle for $f$ with $(\rho,\epsilon)$ random outlier noise. For any point $x$, define $y(x) = f(x) + e(x)$ and let $\Delta$ be an 
 upper bound on $\sum_{i=1}^m |e(x_i)|$ and  $\sigma_{\gap}$ be defined as $\sigma_{\gap}\overset{\text{def}}{=}\Delta-\sum_{i=1}^m |e(x_i)|$.
 {\color{red}{If the points $x_1, \ldots, x_m$ are chosen at random}}, 
then the linear program \eqref{eq:LP_decode_sparseFFT} returns $g$ satisfying 
$$
\E[|f-g|] \le \frac{\sigma_{\gap}}{m \cdot \delta} + \frac{\eps}{\delta} \text{ with probability }1-\gamma.
$$ 
This implies every coefficient $\xi$, $|\wh{f}(\xi)-\wh{g}(\xi)| \lesssim \frac{\sigma_{\gap}}{m \cdot \delta} + \frac{\eps}{\delta}$.
\end{lemma}
Note that the output $g$ of the linear program \eqref{eq:LP_decode_sparseFFT} is not necessarily Fourier sparse. Next, we have the following lemma whose proof is quite similar to that of Lemma~\ref{lem:guarantee_LP}. Note that unlike $g$ in Lemma~\ref{lem:guarantee_LP}, the function $g$ in Lemma~\ref{cor:correctness_over_k_sparse} is not efficiently computable. 
\begin{lemma}\label{cor:correctness_over_k_sparse}
For parameters $\delta>0$ and $\eps>0$ , define $\rho=1/2-\delta$ and $m=\tilde{O} \bigg( k^2 \log |T| \log \frac{1}{\gamma}/\delta^2 \bigg)$.  For $f: D \rightarrow \mathbb{R}$, let $f=\sum_{j=1}^k \wh{f}(\xi_j) \cdot \chi_{j}$ such that  $|\wh{f}(\xi_j)| \ge \frac{5\epsilon}{\delta}$ for all $1 \le i \le k$. For any point $x$, let $y(x)$ be the output of an oracle for $f$ with $(\rho,\epsilon)$ random outlier noise. If the points $x_1, \ldots, x_m$ are chosen at random, 
 then with probability $1-\gamma$, $g=\underset{h:\|\wh{h}\|_0 \le k}{\arg\min} \sum_{i=1}^m |y(x_i)-h(x_i)|$ satisfies
$$
\supp(\wh{g})=\supp(\wh{f}) \text{ and } |\wh{g}(\xi)-\wh{f}(\xi)| \lesssim \frac{\epsilon}{\delta} \text{ for every } \xi.
$$
\end{lemma}

The main technical tool in these proofs is a concentration bound for the following family of functions
\begin{equation}\label{eq:def_FF}
\FF=\left\{ h \big| \supp\{\wh{h}\} \subseteq T, \|\wh{h}\|_1 \le 2 \sqrt{k} \|\wh{h}\|_2 \right\},
\end{equation}
which is a \emph{relaxation} of the family of $2k$-Fourier-sparse functions. The next lemma gives an algorithm for the estimation of $\ell_1$ norm of $h \in \mathcal{F}$. 
\begin{claim}\label{clm:ell_1_ball}
For any $\epsilon$ and failure probability $\gamma$, there exists $m=O\bigg( k^2 \log |T| \cdot \log \frac{1}{\gamma} \cdot \frac{\log^3 \frac{k \log |T|}{\epsilon}}{ \eps^2 }\bigg)$ such that for $m$ random points $x_1,\ldots,x_m \in D$, with probability $1-\gamma$,
$$
\sum_{i=1}^m |h(x_i)| = (1 \pm \epsilon) \cdot m \cdot \E_{x \sim D}\big[ |h(x)| \big] \text{ for any } h \in \mathcal{F}. 
$$ 
\end{claim}

We finish the proof of Theorem~\ref{thm:LP_guarantee_boolean_cube} using Lemma~\ref{lem:guarantee_LP} and Lemma~\ref{cor:correctness_over_k_sparse} here. We defer the proofs of Lemma~\ref{lem:guarantee_LP} and Lemma~\ref{cor:correctness_over_k_sparse} to Section~\ref{sec:supp_proofs_LP} and the proof of Claim~\ref{clm:ell_1_ball} to Section~\ref{sec:proof_ell_1_ball}.

\begin{proofof}{Theorem~\ref{thm:LP_guarantee_boolean_cube}}
We first show that $\sum_{i=1}^m |e(x_i)| \le \sum_i |y(x_i)| + \eps m$. To show this, let $y(x_i) = f(x_i) + e(x_i)$ and $S \subseteq [m]$ denote the subset of queries corrupted by outliers -- i.e., $S = \{i \le m: |e(x_i)| > \epsilon\}$. 

We observe that  with probability $1-\exp(-\delta^2 m)$, the size of $S$ lies  in $[1/2-5\delta/4,1/2-3\delta/4] \cdot m$. Consequently, with probability $1-\exp(-\delta^2 m)$, we also have 
\begin{align*}
\sum_{i \notin S} |y(x_i)| & \ge \sum_{i \notin S} |f(x_i)| - \eps (m-|S|) \\
& \ge (1/2+3\delta/4)m \cdot (1 - \delta/2) \E[|f|] - \eps (m - |S|) \\
& \ge m/2 \cdot \E[|f|] - \eps m.
\end{align*}
Here, the second inequality follows by applying Claim~\ref{clm:ell_1_ball} (with $\epsilon = \delta/2$) to $f$. 






For $\sum_{i \in S} |y(x_i)|$, notice that 
$$
\sum_{i \in S} |e(x_i)| \le \sum_{i \in S} |y(x_i)|+|f(x_i)|,
$$ where $\sum_{i \in S} |f(x_i)| \le |S| \cdot (1+\delta/2) \E[|f|] \le m/2 \cdot \E[|f|]$ by Claim~\ref{clm:ell_1_ball} again. From these discussions, $\sum_{i \notin S} |f(x_i)| \ge \sum_{i \in S} |f(x_i)|$ implies $\sum_{i=1}^m |e(x_i)| \le \sum_i |y(x_i)| + \eps m$.

Hence there exists $\Delta$ in the enumeration of Algorithm~\ref{alg:LP_decoding_boolean} satisfying 
$$
\sum_{i=1}^m |e(x_i)| \le \Delta \le \sum_{i=1}^m |e(x_i)|+\sigma.
$$ 
For such a $\Delta$, by Lemma~\ref{lem:guarantee_LP}, Linear Program \eqref{eq:LP_decode_sparseFFT} returns $g$ satisfying $\underset{x}{\E}[|g(x)-f(x)|] \le \eta/3$ given $\eta \ge \frac{10 \eps}{\delta}$ and our choice of $\sigma$. This implies $|\wh{g}(\xi)-\wh{f}(\xi)| \le \eta/3$ for any $\xi$ and the largest $k$ coefficients in $\wh{g}$ constitute the same set of $\supp(\wh{f})$, i.e., $S_{\Delta}=\supp(\wh{f})$. By Corollary~\ref{cor:correctness_over_k_sparse} over all $k$-Fourier-sparse signals, the final output   $g$ of Algorithm~\ref{alg:LP_decoding_boolean} will have the same support as $\supp(\wh{f})$ satisfying $\E[|f-g|]\lesssim \frac{\eps}{\delta}$.
\end{proofof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
Even though Theorem 3.3 in \cite{RV08} is stated for $k$-Fourier-sparse functions in $T$, its proof works for the relaxation of $\FF$.

\begin{claim}[Restatement of Theorem 3.3 in \cite{RV08}]\label{clm:ell_2_ball}
For any $\epsilon$ and $\gamma$, there exists $m=O\bigg( k \log |T| \cdot \frac{\log \frac{1}{\gamma} \cdot \log^3 \frac{k \log |T|}{\epsilon \cdot \gamma}}{ \eps^2 }\bigg)$ such that for $m$ random points $x_1,\ldots,x_m \in D$, with probability $1-\gamma$,
$$
\sum_{i=1}^m |h(x_i)|^2 = (1 \pm \epsilon) \cdot m \cdot \E\big[ |h(X)|^2 \big] \text{ for any } h \in \mathcal{F}. 
$$ 
\end{claim}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proofs of Lemma~\ref{lem:guarantee_LP} and Corollary~\ref{cor:correctness_over_k_sparse}}\label{sec:supp_proofs_LP}
We first prove Lemma~\ref{lem:guarantee_LP} to show the guarantee of Linear Program~\ref{eq:LP_decode_sparseFFT}.

\begin{proofof}{Lemma~\ref{lem:guarantee_LP}}
Let  $h$ denote $f-g$ and $W$ denote $\supp(\wh{f})$. Since $\|\wh{g}\|_1 \le \|\wh{f}\|_1$, we have
\begin{align*}
\|(\wh{f})_W \|_1 = \|\wh{f}\|_1 & \ge \|\wh{g}\|_1 \\
& \ge \|(\wh{f})_W \|_1 - \|(\wh{h})_W\|_1 + \|(\wh{g})_{\overline{W}}\|_1
\end{align*}
Since $(\wh{g})_{\overline{W}}=(\wh{h})_{\overline{W}}$, This implies $\|(\wh{h})_W\|_1 \ge \|(\wh{h})_{\overline{W}}\|_1$. So $h$ is in the family 
$$
\mathcal{F}_0=\left\{ \|(\wh{h})_W\|_1 \ge \|(\wh{h})_{\overline{W}}\|_1 \bigg| \forall W \in {T \choose k} \right\}.
$$
At the same time, by $\|\wh{h}\|_2 \ge \|(\wh{h})_W\|_2 \ge \frac{1}{\sqrt{|W|}} \|(\wh{h})_W\|_1$ and $|W| \le k$, we have $\FF_0 \subseteq \FF$ for 
$$
\FF=\left\{ h \bigg| \|\wh{h}\|_1 \le 2 \sqrt{k} \cdot \|\wh{h}\|_2 \right\}.
$$

Now we consider the outlier noise. Let $S$ denote the subset of $[m]$ containing outliers. With probability $1-\exp(-\delta^2 n)$, $|S| \le (1/2-3\delta/4)m$. The constraint in \eqref{eq:LP_decode_sparseFFT} indicates
\begin{align*}
\Delta & \ge \sum_i |f(x_i)+e(x_i) - g(x_i)| \\
& = \sum_i |h(x_i)+e(x_i)| \\
& \ge \sum_{i \in S} \left( |e(x_i)|-|h(x_i)| \right) + \sum_{i \in \overline{S}} \left( |h(x_i)|-|e(x_i)| \right)
%\\& = \|e_S\|_1 - \| \big( h(x_1),\ldots, h(x_m) \big)_S \|_1 + \| \big( h(x_1),\ldots, h(x_m) \big)_{\overline{S}} \|_1 -\|e_{\overline{S}}\|_1.
\end{align*}
Since  $\sigma\overset{\text{def}}{=}\Delta-\sum_{i=1}^m |e(x_i)|$, this shows 
\begin{equation}\label{eq:LP_guarantee_under_estimation}
\sigma + 2\sum_{i \in \overline{S}} |e(x_i)|+ \sum_{i \in S} |h(x_i)| \ge \sum_{i \in \overline{S}} |h(x_i)|.
\end{equation}

At the same time, we choose the failure probability in Claim~\ref{clm:ell_1_ball} to be $\gamma/2$ such that with probability $1-\gamma$, we have both
$$
\sum_{i \in S} |h(x_i)| \le (1+\delta/4) \cdot |S| \cdot \E\big[ |h(X)| \big]
$$
and
$$
\sum_{i \in \overline{S}} |h(x_i)| \ge (1 - \delta/4) \cdot |\overline{S}| \cdot \E\big[ |h(X)| \big].
$$
Plugging these two into~\eqref{eq:LP_guarantee_under_estimation} with $|S| \le (1/2-3\delta/4)m$, we have
$$
\sigma + 2\sum_{i \in \overline{S}} |e(x_i)| \ge 0.9 \delta \cdot m \cdot  \E\big[ |h(x)| \big].
$$
Because $|e(x_i)| \le \eps$ for any $i \in \overline{S}$, we have $$
\E[|h(x)|] \le 2 \frac{\sigma}{\delta \cdot m} + 3\frac{\eps}{\delta}.
$$ with probability $1-\gamma$. 

For each $\xi$, $|\wh{f}(\xi)-\wh{g}(\xi)|=|\wh{h}(\xi)| \le \E[|h(x)|]$.
\end{proofof}

Next we prove Corollary~\ref{cor:correctness_over_k_sparse} for $k$-Fourier-sparse functions, whose proof is very similar to the above proof of Lemma~\ref{lem:guarantee_LP}.

\begin{proofof}{Corollary~\ref{cor:correctness_over_k_sparse}}
Suppose $g$ is not equal to the truth $f$. The definition of $g$ implies
$
\sum_{i=1}^m |y(x_i)-g(x_i)| < \sum_{i=1}^m |e(x_i)|.
$

Let $h$ denote $f-g$ and $S$ denote the subset in $[m]$ corrupted by the outlier noise. We have
$$
\sum_{i=1}^m |e(x_i)+h(x_i)| < \sum_{i=1}^m |e(x_i)|.
$$ 
We rewrite the L.H.S. as 
$$
\sum_{i=1}^m |e(x_i)+h(x_i)| \ge \sum_{i \in S} |e(x_i)|-|h(x_i)| + \sum_{i \notin S} |h(x_i)|-|e(x_i)|.
$$ This implies 
\begin{equation}\label{eq:LP_noise_boolean}
\sum_{i \notin S} |h(x_i)| < \sum_{i \in S} |h(x_i)| + 2 \epsilon \cdot (m- |S|).
\end{equation}

At the same time, we have $|S| \le (1/2-3\delta/4) \cdot m$ with probability $1-exp(-\delta^2 \cdot m)$. Since $S$ is independent with $x_1,\ldots,x_m$ and their observations $y(x_1),\ldots,y(x_m)$, wthout loss of generality, we assume $S=\{1,2,\ldots,|S| \}$. Since $h$ is $2k$-sparse, we apply Claim~\ref{clm:ell_1_ball} twice with failure probability $\gamma/2$ to show $h \in \FF$ has 
$$
\sum_{i \in S} |h(x_i)| \le (1+\delta/4) \cdot |S| \cdot \E[|h(X)|] \text{ and } \sum_{i \notin S} |h(x_i)| \ge (1 - \delta/4) \cdot (m-|S|) \cdot \E[|h(X)|].
$$ 
Thus \eqref{eq:LP_noise_boolean} implies
$$
(1-\delta/4) \cdot (1/2+3\delta/4)m \cdot \E[|h(X)|] < (1+\delta/4) \cdot (1/2 - 3\delta/4)m \cdot \E[|h(X)|] + \epsilon \cdot (1+3\delta/2) m.
$$

Thus $\E[|h|] < \frac{2\epsilon}{\delta}$. By definition $h=f-g$ where both $f$ and $g$ are $k$-Fourier-sparse and each coefficient in $f$ has absoulute value $\ge \frac{5\epsilon}{\delta}$, we have $\supp(\wh{g})=\supp(\wh{f})$.
\end{proofof}

\subsection{Proof of Claim~\ref{clm:ell_1_ball}}\label{sec:proof_ell_1_ball}
Without loss of generality,  we can restrict proving Claim~\ref{clm:ell_1_ball} to the subset $ \mathcal{F}_1 \subsetneq \FF$
 $$
\mathcal{F}_1=\left\{ \|\wh{h}\|_1 \le 2\sqrt{k} \bigg| \|\wh{h}\|_2=1 \right\}.
$$ 
We first state two properties for $\FF_1$.
\begin{fact}\label{facts:family_FF}
For any $h \in \FF_1$, we  have
\begin{equation}\label{eq:properties_ell_1_ball}
\max_x |h(x)| \le  2 \sqrt{k} \quad \text{ and } \quad \E_{x \sim D}\big[ |h(x)| \big] \ge \frac{1}{2 \sqrt{k}}.
\end{equation}
\end{fact}
\begin{proof}
First, $\max_x |h(x)| \le \|\wh{h}\|_1 \le 2 \sqrt{k} \|\wh{h}\|_2$. Then $\E_{x \sim D}\big[ |h(x)| \big] \ge \frac{\E_{x \sim D}\big[ |h(x)|^2 \big]}{\max_x |h(x)|} \ge \frac{\|\wh{h}\|^2_2}{2 \sqrt{k} \|\wh{h}\|_2}$.
\end{proof}
We now state the main technical result for  $\FF_1$.
\begin{claim}\label{clm:ell_1_concentration}
There exists $m=O\big( k \log |T| \cdot \log^{3} \frac{k \log |T|}{\eps}/\eps^2 \big) $ such that 
\begin{equation}\label{eq:gaussian_ell_1_ball}
\E_{z_1,\ldots,z_m} \left[ \sup_{h \in \FF_1} \left| \sum_{i=1}^m |h(z_i)| - m \cdot \E_x\big[ |h(x)| \big] \right| \right] \le \epsilon \cdot m. 
\end{equation}
This implies 
$$
\E_{z_1, \ldots, z_m}\left[ \sup_{h \in \FF: \E_{x \sim D}[|h(x)|]=1} \left| \sum_{i=1}^m |h(z_i)| - m  \right| \right] \le \eps \cdot m \text{ for } m = O\bigg( \frac{k^2 \log |T|}{\eps^2} \cdot \log^{3} \frac{k \log |T|}{\eps} \bigg)
$$ by rescaling $\eps$ to $\frac{\eps}{2\sqrt{k}}$ with the lower bound of $ \E_{x \sim D} \big[ |h(x)| \big]$ in \eqref{eq:properties_ell_1_ball}. 
\end{claim}
By Markov's inequality, it implies Claim~\ref{clm:ell_1_ball} with $m = O\bigg( k^2 \log |T| \cdot \log^{3} \frac{k \log |T|}{\gamma \eps} \cdot \frac{1}{\eps^2 \gamma^2} \bigg)$ for any  $\gamma$. It is straightforward to extend Theorem 3.3 in \cite{RV08} to obtain a better dependence of $\log \frac{1}{\gamma}$ on $m$. We use McDiarmid's inequality to provide an alternative argument. 
\begin{lemma}[McDiarmid's inequality \cite{McDiarmid:89}]
Let $F$ be a function which is $c_i$-Lipschitz in the $i^{th}$ direction. In other words, 
 $$ \underset{x_1,\ldots,x_n,x'_i}{\sup} \big|F(x_1,\ldots,x_n)-F(x_1,\ldots,x_{i-1},x'_i,x_{i+1},x_n) \big| \le c_i, $$ for each $i \in [n]$. Then, for any $\eps>0$,
$$
\Pr_{z_1, \ldots, z_n \sim D}\bigg[|F(z_1,\ldots,z_n)-\E_{x}[F(x_1,\ldots,x_n)]| \ge \eps \bigg] \le 2\exp\left( -\frac{2\eps^2}{\sum_{i=1}^n c_i^2} \right).
$$
\end{lemma}

\begin{proofof}{Claim~\ref{clm:ell_1_ball}}
Given $z_1,\ldots,z_n$, we define $F(z_1,\ldots,z_n)$ to be $$
\sup_{h \in \FF: \E[|h|]=1} \left| \sum_{i=1}^m |h(z_i)| - m  \right|.
$$
Notice that for any $z_i,z'_i \in D$, Fact~\ref{facts:family_FF} shows
$$
|F(z_1,\ldots,z_n)-F(z_1,\ldots,z_{i-1},z'_i,z_{i+1},z_n)| \le \sup_{h \in \FF: \E[|h|=1]} \sup_{x} |h(x)| \le 4k.
$$
Choosing  $m=O\bigg( \log \frac{1}{\gamma} \cdot k^2 \log |T| \cdot \log^{3} \frac{k \log |T|}{\eps}/\eps^2 \bigg)$ implies (using Claim~\ref{clm:ell_1_concentration}) that 
$$
\E[F(x_1,\ldots,x_m)] \le \eps \cdot m.
$$
Then, McDiarmid's inequality implies
$$
\Pr\left[\bigg|F(x_1,\ldots,x_m) - \E[F(x_1,\ldots,x_m)] \bigg| \ge a \right] \le 2 \exp\left(-\frac{2a^2}{(4k)^2 \cdot m}\right).
$$
For $a=\eps m$, this is at most $\gamma$. We rescale $\eps$ to finish the proof.
\end{proofof}
Thus, it remains to prove Claim~\ref{clm:ell_1_concentration} -- to do this, we use a standard symmetrization and Gaussianization argument~\cite{LTbook} which transforms bounding the left hand side of \eqref{eq:gaussian_ell_1_ball} to bounding a Gaussian process. In particular, we will use the following theorem (whose proof, for 
completeness, is provided in Appendix~\ref{appd:sym_gau}). 

\define{thm:sym_gauss}{Theorem}{ Let $X$ be a random variable and $S$ be a set of events. Let $\bx= (x_1, \ldots, x_n)$ and $\bx'=(x'_1, \ldots, x'_n)$ be independent samples from $\bX^n$.
Let $\boldsymbol{g}=(g_1,\cdots,g_n)$ be sampled from the standard $n$-dimensional normal $N(0,1)^n$. Then, for any non-negative function $f: S \times \supp(X) \rightarrow \mathbb{R}^+$ ,
$$
\underset{\bx}{\E}\left[\max_{\Lambda \in S} \left|\sum_{j=1}^n f(\Lambda,x_j) - \underset{\bx'}{\E}[\sum_{j=1}^n f(\Lambda,x'_j)] \right|\right] \le \sqrt{2\pi} \cdot \underset{\bx}{\E} \left[ \underset{\bg}{\E}\left[\max_{\Lambda \in S} \left|\sum_{j=1}^n f(\Lambda,x_j) g_j\right| \right] \right].
$$}
\state{thm:sym_gauss}

Then we relax the L.H.S. of \eqref{eq:gaussian_ell_1_ball} to
$$
\sqrt{2 \pi} \cdot \E_{x_1,\ldots,x_m \sim D} \E_{\boldsymbol{g}\sim N(0,1)^m} \left[ \sup_{h \in \FF_1} \left| \left \langle \big( |h(x_i)| \big)_{i \in [m]}, \boldsymbol{g} \right \rangle \right| \right]. 
$$ 
In the rest of this section, we bound the Gaussian process using Dudley's entropy integration.

We extend Lemma 3.7 in \cite{RV08} to bound the covering number of $\FF_1$. We use $N(S,\|\cdot\|_2,u)$ for a set $S \subseteq \mathbb{R}^m$ to denote its covering under Euclidean distance of radius $u$ --- the minimum size of $T \subseteq \mathbb{R}^m$ such that for any $v \in S$, there exists $v' \in T$ satisfying $\|v-v'\|_2 \le u$.

\begin{claim}\label{clm:covering_ell_1_ball}
Given any $x_1,\ldots,x_m \in D$, radius $u$, and $l$, the covering number
$$
N \left( \bigg\{ \big( |h(x_i)| \big)_{i \in [m]} \bigg| \|\wh{h}\|_1 \le l \bigg\}, \| 
\cdot \|_{2},u \right) \le |T|^{O(m \cdot \log m \cdot \frac{l^2}{u^2})}.
$$
\end{claim}
\begin{proof}
For $h,h' \in \FF_1$, the $\ell_2$ distance of corresponding vectors is
$$
\left(\sum_{i \in [m]} \left( |h(x_i)| - |h'(x_i)| \right)^2 \right)^{1/2} \le \left( \sum_{i \in [m]} \bigg( h(x_i) - h'(x_i) \bigg)^2 \right)^{1/2} \le \sqrt{m} \cdot \max_{i \in [m]} \bigg| h(x_i) - h'(x_i) \bigg|.
$$
So $$N \left( \bigg\{ \bigg( |h(x_i)|  \bigg)_{i \in [m]} \bigg| \|\wh{h}\|_1 \le l  \bigg\}, \| \cdot \|_{2},u \right) \le N \left(\bigg\{  \bigg( h(x_i) \bigg)_{i \in [m]} \bigg| \|\wh{h}\|_1 \le l \bigg\}, \| \cdot \|_{\infty}, \frac{u}{\sqrt{m}} \right)$$

By rescaling the $\ell_1$ norm of the family, it is enough to prove 
$$
N \left( \left\{ \bigg( h(x_i)  \bigg)_{i \in [m]} \bigg| \|\wh{h}\|_1 \le 1 \right \}, \| \cdot \|_{\infty},u \right) \le (2|T|)^{\frac{C \log m }{u^2}} \text{ for } C=O(1).
$$

Given any $h$ with $\|\wh{h}\|_1=1$, we define a random vector $Z \in \mathbb{R}^{|T|}$ that takes values 

$$\bigg(0,\ldots,0,sign\big(\wh{h}(\xi) \big),0,\ldots,0 \bigg) \text{ with prob. } |\wh{h}(\xi)| 
$$ 
for each $\xi$ with nonzero coefficient $\wh{h}(\xi)$. Let $Z_1,\ldots,Z_t$ be i.i.d. copies of $Z$ for $t=C \cdot \log m /u^2$ with some large constant $C$.	Notice that $$\E Z = \wh{h} \text{ and } \E \wh{Z} = h.$$ 

We plan to bound
\begin{equation}\label{eq:sym_gau_Z}
\E_{Z_1,\ldots,Z_t}\bigg[ \sup_{j \in [m]}\bigg| \frac{1}{t} \sum_{i \in [t]} \wh{Z_i}(x_j)  - \E\big[ \wh{Z}(x_j) \big] \bigg|\bigg] \lesssim \sqrt{\frac{\log m}{t}}.
\end{equation} 
This will indicate $\exists z_1,\ldots,z_t \in \supp(Z)$ such that $\sup_{j \in [m]}\bigg| \frac{1}{t} \sum_{i \in [t]} \wh{z_i}(x_j)  - h(x_j) \bigg| \le u$ from the choice $t=C \cdot \log m /u^2$.

We apply Theorem~\ref{thm:sym_gauss} of symmetrization and Gaussianization on the L.H.S. of \eqref{eq:sym_gau_Z}:
$$
\E_{Z_1,\ldots,Z_t}\bigg[ \sup_{j \in [m]}\bigg| \frac{1}{t} \sum_{i \in [t]} \wh{Z_i}(x_j)  - \E\big[ \wh{Z}(x_j) \big] \bigg|\bigg] \lesssim \frac{1}{t} \cdot \E_{Z_1,\ldots,Z_t} \E_{g} \left[ \sup_{j \in [m]} \bigg| \sum_{i \in [t]} g_i \cdot \wh{Z_i}(x_j) \bigg| \right].
$$

For each $j$, $\sum_{i \in [t]} g_i \cdot \wh{Z_i}(x_j)$ is a Gaussian random variable with variance $ t \cdot 1$. For the maximum over $m$ Gaussian random variables with variance $t$, $\E_{g} \left[ \sup_{j \in [m]} \bigg| \sum_{i \in [t]} g_i \cdot \wh{Z_i}(x_j) \bigg| \right] \lesssim \sqrt{t \cdot \log m}$ from Lemma~\ref{lem:Gaussian_variables}, which proves \eqref{eq:sym_gau_Z} after the normalization $1/t$.

Because there are $2 \cdot |T|$ choices for each $Z_i$, this bounds 
$$
N \left( \left\{ \bigg( h(x_i)  \bigg)_{i \in [m]} \bigg| \|\wh{h}\|_1 \le 1 \right \}, \| \cdot 	\|_{\infty},u \right) \le (2 \cdot |T|)^{t} = (2 \cdot |T|)^{O(\log m /u^2)}.
$$
\end{proof}

\begin{claim}
Given any $x_1,\ldots,x_m$, 
$$
\E_{\boldsymbol{g}} \left[ \sup_{h \in \FF_1} \left| \left \langle \big( |h(x_i)| \big)_{i \in [m]}, \boldsymbol{g} \right \rangle \right| \right] \lesssim \sqrt{m k \log |T| } \cdot \log^{1.5} m.
$$
\end{claim}
\begin{proof}
We apply Dudley's entropy integration to bound the Gaussian process:
$$
\E_{\boldsymbol{g}} \left[ \sup_{h \in \FF_1} \left| \left \langle \big( |h(x_i)| \big)_{i \in [m]}, \boldsymbol{g} \right \rangle \right| \right] \le \int_{0}^{2\sqrt{km}} \sqrt{\log N\left( \left\{ \big( |h(x_j| \big)_{j \in [m]} \big| h \in \FF_1 \right\}, \|\cdot\|_2,u\right)} \mathrm{d} u.
$$
For $u$ from $0$ to $1$, we use a covering of size $(\frac{2\sqrt{k \cdot m}}{u} )^{m}$  because $\big( |h(x_j| \big)_{j \in [m]} \in \bigg[ 0,2\sqrt{k} \bigg]^{m}$. Next we use the covering in Claim~\ref{clm:covering_ell_1_ball} to bound the integreation from $u=1$ to $2\sqrt{m \cdot k}$:
\begin{align*}
& \int_{0}^{1} \sqrt{\log  (\frac{2\sqrt{k \cdot m}}{u} )^{m} } \mathrm{d} u + 
\int_{1}^{2\sqrt{km}} \sqrt{\log C^{ \log |T| \cdot m \cdot \log m \cdot \frac{k}{u^2} } } \mathrm{d} u\\
 \lesssim & \int_0^{1} \sqrt{m \cdot \log \sqrt{k m} + m \log 1/u} \mathrm{d} u + \int_{1}^{2\sqrt{km}} \sqrt{\log |T| \cdot m \cdot \log m \cdot \frac{k}{u^2} } \mathrm{d} u\\
 \lesssim & \sqrt{m k \log |T|} \cdot \log^{1.5} m.
\end{align*}
\end{proof}
Claim~\ref{clm:ell_1_concentration} follows from the above bound with $m=C \cdot \frac{k \log |T| \cdot \log^3 (k \log |T|/\eps) }{\eps^2}$ for a constant $C$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
